CustomKD: Customizing Large Vision Foundation for Edge Model Improvement via Knowledge Distillation

We propose a novel knowledge distillation approach, CustomKD, that effectively leverages large vision foundation models (LVFMs) to enhance the performance of edge models (e.g., MobileNetV3). Despite recent advancements in LVFMs, such as DINOv2 and CLIP, their potential in knowledge distillation for enhancing edge models remains underexplored. While knowledge distillation is a promising approach for improving the performance of edge models, the discrepancy in model capacities and heterogeneous architectures between LVFMs and edge models poses a significant challenge. Our observation indicates that although utilizing larger backbones (e.g., ViT-S to ViT-L) in teacher models improves their downstream task performances, the knowledge distillation from the large teacher models fails to bring as much performance gain for student models as for teacher models due to the large model discrepancy. Our simple yet effective CustomKD customizes the well-generalized features inherent in LVFMs to a given student model in order to reduce model discrepancies. Specifically, beyond providing well-generalized original knowledge from teachers, CustomKD aligns the features of teachers to those of students, making it easy for students to understand and overcome the large model discrepancy overall. CustomKD significantly improves the performances of edge models in scenarios with unlabeled data such as unsupervised domain adaptation (e.g., OfficeHome and DomainNet) and semi-supervised learning (e.g., CIFAR-100 with 400 labeled samples and ImageNet with 1% labeled samples), achieving the new state-of-the-art performances.

==> tables/main_semi_total.tex <==
\begin{table*}[!t]
    \begin{minipage}{.45\linewidth}
      \centering
        \scalebox{0.85}{
        \begin{tabular}{c|c|ccc} 
        \toprule
        \multirow{2}{*}{Category} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Labels} \\ 
         & & 400 \hfill & 2500 \hfill & 10000 \hfill \\ 
        \drule
         % & DINO-V2~\cite{dinov2}	                & 17.92 & 11.49 & 9.13 \\
         % & Supervised*~\cite{wide_resnet}	    & 28.20 & 28.20 & 28.20 \\
         % \midrule
        \multirow{6}{*}{SSL} & FixMatch~\cite{fixmatch}	        & 53.37 & 34.29 & 28.28 \\
        & SimMatch~\cite{simmatch}	        & 48.82 & 32.54 & 26.42 \\
        & FreeMatch~\cite{freematch}	    & 49.24 & 32.79 & 27.17 \\
        & SoftMatch~\cite{softmatch}	    & 49.64 & 33.05 & 27.26 \\
        % & AdaMatch~\cite{adamatch}	    & 47.82 & 33.26 & 27.53 \\
        % \cmidrule{2-5}
        & AdaMatch*~\cite{adamatch}	    & 52.07 & 37.92 & 32.5 \\
        \midrule
        \multirow{7}{*}{KD} & Soft Target~\cite{soft_target} & 48.71 & 31.73 & 27.66 \\
        & Logits~\cite{logits} & 49.71 & 33.42 & 28.16 \\
        & DKD~\cite{decoupled_kd} & 45.18 & 30.43 & 26.19 \\        
        & RKD~\cite{rkd} & 50.11 & 34.24 & 29.11 \\
        & CC~\cite{cc} & 49.85 & 33.72 & 28.75 \\
        & FitNet~\cite{fitnet} & 48.58 & 30.87 & 29.41 \\
        & \cellcolor{Gray}Ours & \cellcolor{Gray}\textbf{32.51} & \cellcolor{Gray}\textbf{25.52} & \cellcolor{Gray}\textbf{24.66} \\
        \bottomrule
        \end{tabular}}
        \vspace{0.05cm}
      \caption{Error rates of semi-supervised learning on CIFAR-100. * indicates reproduced results using codes of USB benchmark.}
      \label{tab:main_semi_cifar100}
    \end{minipage}%
    \hfill \hfill \hfill
    \begin{minipage}{.45\linewidth}
      \centering
        \scalebox{0.85}{
        \begin{tabular}{c|cc|cc} 
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Top-1} & \multicolumn{2}{c}{Top-5} \\ 
         & 1\% & 10\% & 1\% & 10\% \\ 
        \drule
        Vat + EntMin~\cite{vat,minentp}	        &  - & 68.8 & -	& 88.5 \\
        S4L-Rotation~\cite{s4l}                 & -	 & 53.4 & -	& 83.8 \\ 
        UDA~\cite{UDA}                          & -	 & 68.8 & -	& 88.5 \\
        FixMatch~\cite{fixmatch}	            & -    & 71.5 & -	& 89.1 \\
        CoMatch~\cite{CoMatch}	                & 66.0 & 73.6 & 86.4 & 91.6 \\
        SimMatch~\cite{simmatch}	            & 67.2 & 	74.4 & 87.1	& 91.6 \\
        \cellcolor{Gray}Ours        & \cellcolor{Gray}\textbf{67.5} & 	\cellcolor{Gray}\textbf{74.7} & \cellcolor{Gray}\textbf{87.6} & \cellcolor{Gray}\textbf{91.9} \\        
        \bottomrule
        \end{tabular}}
        \vspace{0.05cm}
      \caption{Image classification accuracy of semi-supervised learning on Imagenet.}
      \label{tab:main_semi_imagenet}
    \end{minipage} 
    \vspace{-0.4cm}
  \label{tab:main_semi_total}
\end{table*}




==> tables/rebuttal_ablation_epoch.tex <==

{\renewcommand{\arraystretch}{.97}
\begin{table}[h]
\centering
\begin{center}
{
\resizebox{0.45\textwidth}{!}{
{
\begin{tabular}{cc|cccccc} 
\toprule
\multicolumn{2}{c|}{Method} & OpenCLIP-B & OpenCLIP-L & EVA02-B & EVA02-L & DINOv2-S & DINOv2-L \\ 
\drule

\multicolumn{2}{c|}{FitNet} & 57.32 & 57.85 & 56.16 & 56.01 & 70.69 & 71.94  \\
\midrule
            & 30:1   & 61.90 & 64.50 & 61.02 & 63.90 & 70.74 & 73.76  \\
CustomKD    & 10:1   & 62.32 & 64.64 & 62.06 & 64.71 & \textbf{70.75} & 73.74 \\
Alternation & 5:1    & 62.54 & 64.64 & 62.46 & \textbf{65.09} & 70.67 & \textbf{73.86}  \\
            & 1:1    & \textbf{62.66} & \textbf{64.82} & \textbf{62.61} & 65.03 & 70.72 & 73.78  \\

\bottomrule
\end{tabular}}}}
\end{center}
\end{table}
}




==> tables/rebuttal_ablation_loss.tex <==
{\renewcommand{\arraystretch}{.97}
\begin{table}[h]
  \centering
    \vspace{-0.35cm}
    \scalebox{0.55}{
    \begin{tabular}{c|cc|cc|cc|cc} 
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{OpenCLIP-B} & \multicolumn{2}{c|}{OpenCLIP-L} & \multicolumn{2}{c|}{DINOv2-S} & \multicolumn{2}{c}{DINOv2-L} \\ 
     & Acc. & CKA & Acc. & CKA & Acc. & CKA & Acc. & CKA \\ 
    \drule
    Without KD	                     & 49.52 & - & 49.52 & -  & 49.52 & -  & 49.52 & - \\
    $\mathcal{L}_{f_{t}}$	         & 50.14 & 0.2704 & 50.83 & 0.2058 & 66.59 & 0.6870 & 65.78 & 0.5670 \\
    $\mathcal{L}_{\tilde{f_{t}}}$    & 55.31 & 0.5942 & 56.92 & 0.6082 & 56.71 & 0.6219 & 58.27 & 0.5851 \\
    $\mathcal{L}_{f_{t}}$ + $\mathcal{L}_{\tilde{f_{t}}}$ & \textbf{56.08} & \textbf{0.6050} & \textbf{58.43} & \textbf{0.6170} & \textbf{67.34} & \textbf{0.7106} & \textbf{69.25} & \textbf{0.6698} \\
    \bottomrule
    \end{tabular}
    }
\vspace{-0.4cm}
\end{table}
}


% {\renewcommand{\arraystretch}{.97}
% \begin{table}[b]
%   \vspace{-0.6cm}
%   \centering
%     \scalebox{0.52}{
%     \begin{tabular}{c|ccc|ccc|ccc|ccc} 
%     \toprule
%     \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{OpenCLIP-B} & \multicolumn{3}{c|}{OpenCLIP-L} & \multicolumn{3}{c|}{DINOv2-S} & \multicolumn{3}{c}{DINOv2-L} \\ 
%      & Acc. & CKA & Time & Acc. & CKA & Time & Acc. & CKA & Time & Acc. & CKA & Time \\ 
%     \drule
%     Min Entp.	                     & 49.52 & - & xx.xx & 49.52 & - & xx.xx  & 49.52 & - & xx.xx  & 49.52 & - & xx.xx \\
%     $\mathcal{L}_{f_{t}}$	         & 50.14 & 0.2704 & xx.xx & 50.83 & 0.2058 & xx.xx  & 66.59 & 0.6870 & xx.xx  & 65.78 & 0.5670 & xx.xx  \\
%     $\mathcal{L}_{\tilde{f_{t}}}$    & 55.31 & 0.6371 & xx.xx & 56.92 & 0.6436 & xx.xx  & 56.71 & 0.6784 & xx.xx  & 58.27 & 0.6534 & xx.xx  \\
%     $\mathcal{L}_{f_{t}}$ + $\mathcal{L}_{\tilde{f_{t}}}$ & \textbf{56.08} & \textbf{0.6458} & xx.xx & \textbf{58.43} & \textbf{0.6595} & xx.xx  & \textbf{67.34} & \textbf{0.7509} & xx.xx & \textbf{69.25} & \textbf{0.7237} & xx.xx  \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table}
% }

==> tables/rebuttal_hyperparams.tex <==

{\renewcommand{\arraystretch}{.97}
\begin{table}[h]
\centering
\begin{center}
{
\resizebox{0.45\textwidth}{!}{
{
\begin{tabular}{ccccc} 
\toprule
LR & Batch Size & Epochs & $\lambda_{U}$ & $\lambda_{kd}$ \\ 
\midrule
0.01 & 32 & 60 & 0.1 & \{0.1, 1.0, 10.0, 100.0\} \\

\bottomrule
\end{tabular}}}}
\end{center}
\end{table}
}

==> tables/rebuttal_pred.tex <==
{\renewcommand{\arraystretch}{.97}
\begin{table}[h]
\centering
\begin{center}
{
\resizebox{0.35\textwidth}{!}{
{
\begin{tabular}{c|ccc|c} 
\toprule
Method & CIFAR400 & CIFAR2500 & CIFAR10000 & Avg. \\ 
\drule

WRN28-2 & 90.35 & 69.73 & 49.6 & 69.89  \\
\midrule
Soft Target  & 66.67 & 61.77 & 41.81 & 56.75  \\
+ Ours       & 42.60 & 32.69 & 28.33 & 34.54  \\
% \midrule
% DKD          & 54.51 & 57.19 & 39.19 & 50.30  \\
% + Ours       & 41.22 & 31.15 & 27.52 & 33.30  \\

\bottomrule
\end{tabular}}}}
\end{center}
\vspace{-0.4cm}
\end{table}
}

==> tables/rebuttal_time.tex <==

{\renewcommand{\arraystretch}{.97}
\begin{table}[h]
\centering
\begin{center}
{
\resizebox{0.39\textwidth}{!}{
{
\begin{tabular}{c|cccc} 
\toprule
Method & OpenCLIP-B & OpenCLIP-L & DINOv2-S & DINOv2-L \\ 
\drule
Without KD   & 0.05 & 0.05 & 0.05 & 0.05 \\ 
\midrule
FitNet      & 0.23 & 0.92 & 0.13 & 0.92 \\
CustomKD    & 0.25 & 0.95 & 0.14 & 0.98 \\

\bottomrule
\end{tabular}}}}
\end{center}
\end{table}
}
